Covering Tours and Cycle Covers with Turn Costs: Hardness and Approximation

We investigate a variety of problems of finding tours and cycle covers with minimum turn cost. Questions of this type have been studied in the past, with complexity and approximation results as well as open problems dating back to work by Arkin et al. in 2001. A wide spectrum of practical applications have renewed the interest in these questions, and spawned variants: for full coverage, every point has to be covered, for subset coverage, specific points have to be covered, and for penalty coverage, points may be left uncovered by incurring an individual penalty. We make a number of contributions. We first show that finding a minimum-turn (full) cycle cover is NP-hard even in 2-dimensional grid graphs, solving the long-standing open Problem 53 in The Open Problems Project edited by Demaine, Mitchell and O'Rourke. We also prove NP-hardness of finding a subset cycle cover of minimum turn cost in thin grid graphs, for which Arkin et al. gave a polynomial-time algorithm for full coverage; this shows that their boundary techniques cannot be applied to compute exact solutions for subset and penalty variants. On the positive side, we establish the first constant-factor approximation algorithms for all considered subset and penalty problem variants, making use of LP/IP techniques. For full coverage in more general grid graphs (e.g., hexagonal grids), our approximation factors are better than the combinatorial ones of Arkin et al. Our approach can also be extended to other geometric variants, such as scenarios with obstacles and linear combinations of turn and distance costs.

==> 96_formal_definition.tex <==
\section{Formal Problem Definition}
\label{sec:apdx:problems}
For easier reference, we provide a full set of formal definitions. I case of acceptance, these will be 
contained in a full version of the paper, to be posted at the arXiv.

\subsection{Grid Graphs}
In the followin, we formalize the different problem variants.
We focus on 2-dimensional grid graphs; the generalization to other grids is straightforward.

%Definition cycle

\begin{definition}[Cycle]
	A {\em cycle} in a 2-dimensional grid graph $G(V,E)$ is a sequence of pixel/vertices $v_0, v_1, \ldots, v_n\in V$ with $v_0=v_n$ and $\forall v_i, v_{i+1}: \{v_i, v_{i+1}\}\in E$.
	It has length $n\geq 2$, which equals the number of transitions.
\end{definition}
Note that a pixel can be visited multiple times by a cycle. We acquire at least two distinct pixels in a cycle to prevent degeneracies.
%We can allow cycles with only one pixel in it, but the meaning of them would be odd so that we prohibit them.
%However, most of the results in this paper would actually allow the integration of such cycles.

%Cost of cycle
The {\em cost} of a cycle consists of two parts: costs for each turn and costs for each pixel transition (or its length).
We also refer to these costs as {\em turn costs} and {\em distance costs}.
There are three different possible turns: $+90\degree$, $-90\degree$, and $180\degree$.
We count $+90\degree$ and $-90\degree$ as a single turn.
while u-turns of $180\degree$ incur a cost of two simple turns.
We get analogous values for a hexagonal grid, with turns of $\pm 60\degree$, $\pm 120\degree$, and $180\degree$ turns and incurring a cost of one turn, two turns, and three turns, respectively.

A transition from one pixel to an adjacent pixel adds $1$ to the length of the tour.
The cost of a cycle is a linear combination of the number of turns and its length:
for a cycle $\gamma$ of length $s$ and $t$ has a cost $c_{\kappa,\tau}(\gamma)=s*\kappa+t*\tau$, with $\kappa\in\mathbb{R}^+_0$ and $\tau\in\mathbb{R}^+_0$ being two appropriate constants. (Thus, a cycle that only covers two adjacent pixels has a turn cost of $4$ and a length of $2$.)

We now consider the details of the different variants.

%-------------------------------------------------------------------------------------------
% 2D-Milling
%-------------------------------------------------------------------------------------------
\subsubsection{Full Coverage}

The simplest problem variants are {\em full coverage cycle cover} and {\em full coverage tour cover},
where it every pixel has to be covered by a cycle cover or a tour, respectively.
%A realistic scenario of such a full coverage tour could be the harvesting of a field and the milling or scanning of an area.
%For our example with the mosquito hunting drone in the motivation, it could be useful if no expected mosquito distributions are known.

%Formal Problem Definitions
\begin{problem}[Full cycle cover]
	\label{prob:2dcc}
	Given a connected grid graph $G=(V,E)$ and two weights $\kappa,\tau\in \mathbb{R}^+_0$.
	Find a set of cycles $\mathcal{C}=\{\pi_0,\pi_1, \ldots\}$ such that every vertex $v\in V$ is visited at least once by some cycle of $\mathcal{C}$ and $\sum_{\pi_i \in \mathcal{C}}c_{\kappa,\tau}(\pi_i)$ is minimal.
\end{problem}

A cycle cover is a tour if it only contains a single cycle.
\begin{problem}[Full tour]
	\label{prob:2dtour}
	Given a connected grid graph $G=(V,E)$ and two weights $\kappa,\tau\in \mathbb{R}^+_0$.
	Find a single closed cycle (a {\em tour} $\pi$ in $G$, such that every vertex $v\in V$ is visited at least once, 
and $c_{\kappa,\tau}(\pi)$ is minimized.
\end{problem}

%Previous Work
%If we only have distance costs (i.e., $\tau=0$ and $\kappa>0$), the cycle cover can efficiently be calculated by a 2-factor reduction and the tour variant equals the \emph{traveling salesman problem in grid graphs} for which there is a 6/5-approximation by Arkin, Fekete, and Mitchell~\cite{arkin2000approximation}.
%The variant with turn costs has already been considered by Arkin et al.~\cite{arkin2005optimal, arkin2001optimal}, Maurer~\cite{maurer2009diploma}, and de Assis and de Souza~\cite{de2011experimental}.

%-------------------------------------------------------------------------------------------
% subset Milling
%-------------------------------------------------------------------------------------------
\subsubsection{Subset Coverage}

%Motivation for subset coverage
If we only need to visit a subset of pixels,
%A practical variation of the previous problem might be that only a subset of the pixel has to be visited.
%In case of our drone example, this might be the pixel where the mosquito swarms are expected.
%All other pixel are just feasible positions but without any direct advantages (except for possibly providing a short way to another important position).
we get problem variations similar to the \emph{Steiner tree on graphs} as a variation of the \emph{minimum spanning tree}.
%; see the book of Hwang et al.~\cite{hwang1992Steiner} for an overview of the Steiner tree problem.

%Definition
\begin{problem}[Subset cycle cover]
	\label{prob:gg:subsetcc}
	Given a connected grid graph $G=(V,E)$, a set $S\subseteq V$, and two weights $\kappa,\tau\in \mathbb{R}^+_0$.
	Find a set of cycles $\mathcal{C}=\{\pi_0,\pi_1, \ldots\}$ such that every vertex $v\in S$ is visited at least once by some cycle of $C$, and $\sum_{\pi_i \in \mathcal{C}}c_{\kappa,\tau}(\pi_i)$ is minimized.
\end{problem}
And the respective tour version of the problem:
\begin{problem}[Subset tour]
	\label{prob:subsettour}
	Given a connected grid graph $G=(V,E)$, a set $S\subseteq V$, and two weights $\kappa,\tau\in \mathbb{R}^+_0$.
	Find a tour/cycle $\pi$ in $G$ such that every vertex $v\in S$ is visited at least once, and $c_{\kappa,\tau}(\pi)$ is minimized.
\end{problem}

%Model Full coverage
For $V=S$, Problem~\ref{prob:gg:subsetcc} and Problem~\ref{prob:subsettour} are equivalent to Problem~\ref{prob:2dcc} and Problem~\ref{prob:2dtour}, respectively.

\subsubsection{Penalty Coverage}

%Motivation for penalty coverage
Another natural generalization arises from covering pixels with different values or densities.
%In the case of the example with the drone, the previous variation allowed us to only enforce the lucrative pixel to be covered.
%A natural extension of this is to not to force visiting lucrative pixel but to give a prize for it.
%This can also be seen as a penalty for not visiting these pixel.
%Some pixel might be lucrative but very far away from the other lucrative pixels and an integration of them might not be reasonable.
%This new problem formulation allows the tour to actually skip these pixel with a bad usage/cost-ratio while the previous formulation would have enforced an additional expensive preoptimization which is also inaccurate because the costs depend on the actual tour.
%
%TSP
This is similar to the \emph{penalty traveling salesman problem~(PTSP)} variation of the TSP.
For the PTSP, a 2-approximation is known for the case that the triangulation inequality holds for the corresponding graph~\cite{goemans1995general}.
The PTSP is often also wrongly called the \emph{prize-collecting traveling salesman problem (PCTSP)} but the PCTSP also contains a quota that has to be fulfilled, see~\cite{ausiello2007prize}.
%\todoi{This last reference is only used here in the appendix.}
%For the PCTSP only a $O(\log^2(\min(Q,n)))$-approximation algorithm by Awerbuch et al.~\cite{awerbuch1998new} is known to us where $Q$ is the quota.
%PTSP and PCTSP both have only distance costs and no turn costs.

%Definition
The definitions of cycle cover and tour variants can be given as follows.
\begin{problem}[Penalty cycle cover]
	Given a connected grid graph $G=(V,E)$, a penalty function $\rho:V\rightarrow \mathbb{R}^+_0$, and two weights $\kappa,\tau\in \mathbb{R}^+_0$.
	Find a set of cycles $\mathcal{C}=\{\pi_0,\pi_1, \ldots\}$, such that $\sum_{\pi_i \in \mathcal{C}}c_{\kappa,\tau}(\pi_i)+\sum_{v\in V\setminus V(\mathcal{C})} \rho(v)$ is minimized,
	where $V(\mathcal{C})$ denotes the pixel covered by $\mathcal{C}$.
\end{problem}

\begin{problem}[Penalty tour]
	Given a connected grid graph $G=(V,E)$, a penalty function $\rho:V\rightarrow \mathbb{R}^+_0$, and two weights $\kappa,\tau\in \mathbb{R}^+_0$.
	Find a tour/cycle $\pi$ in $G$, such that $c_{\kappa,\tau}(\pi)+\sum_{v\in V\setminus V(\pi)}\rho(v)$ is minimized.
\end{problem}

%PTSP sometimes has root
In some scenarios, the PTSP is defined with a root vertex that has to be covered;
this can be modeled in our formulation by setting the penalty for the root pixel sufficiently high.
%Model subset coverage
Similarly, the penalty coverage problem can model the subset coverage problem by using a high penalty for the pixels in the subset.
%This high penalty could, e.g., be the cost of a greedily computed tour.

\subsection{Geometric Versions}
%Cycle Definition
We can generalize the previous definitions to more general geometric versions.
%While the discretization of the passing orientations allows us to provide simple constant factor approximation algorithms (for fixed discretization resolution), the definition of the costs of a cycle becomes more complicated compared to the non-discretized version.
We express a cycle as a sequence of configurations (position and heading).
A point $p$ with the discretized orientations $\delta(p)$ is covered by a cycle if one of its configurations $\{(p, \alpha), (p,\alpha+\pi) \mid \alpha \in \delta(p)\}$ is in the cycle.
The transition between two subsequent such configurations equals the optimal transition and the cost of the cycle is the sum of the cost of these transitions.
\begin{definition}
	A {\em cycle} $C$ for a set of points $P$ with the discrete orientations $\delta: P\rightarrow \mathcal{P}([0,\pi))$ in a polygonal environment with the obstacles $\mathcal{O}$ is a sequence of configurations $\sigma_0=(p_0\in P, \alpha_0\in \{\alpha, \alpha+\pi \mid \alpha \in \delta(p_0)\}), \ldots, \sigma_n=(p_n\in P, \alpha_n\in \{\alpha, \alpha+\pi \mid \alpha \in \delta(p_n)\})$ with $\forall i=0,\ldots, n-1: p_i\not= p_{i+1}$.
	The cost $c_{\mathcal{O},\kappa, \tau}( C)$ of a cycle is the sum of minimum-cost transitions between any two subsequent configurations
	\[c_{\mathcal{O}, \kappa, \tau}(C) = \text{SP}_{\mathcal{O}, \kappa, \tau}(c_n, c_0)+\sum_{i=0,\ldots, n-1} \text{SP}_{\mathcal{O}, \kappa, \tau}(c_i, c_{i+1}),\]
	where $\text{SP}_{\mathcal{O}, \kappa, \tau}(c_a, c_b)$ denotes the minimum-cost transition (shortest path) from configuration $c_a$ to $c_b$ around the obstacles $\mathcal{O}$ with distance cost parameter $\kappa$ and the turn cost parameter $\tau$.
	If no such transition exists, we assume the cost to be infinite.

	Moreover, for a point $p\in P$ and a cycle $C$, we denote $p\in C \Longleftrightarrow \exists \beta \in \{\alpha, \alpha+\pi \mid \alpha \in \delta(p)\}: (p, \beta)\in C$ as $p$ being covered by $C$.
\qed
\end{definition}

%The computation of the minimum cost transitions/paths in 2D can be done efficiently by utilizing that, analogous to minimizing only the distance, such a path only makes turns at the vertices of obstacles.
%As every discrete orientation consists of two opposing headings, the cycle is symmetric, i.e., it is identical to the reversed configuration sequence with every heading rotated by $180\degree$.
%An alternative definition of such a cycle could be to represent every discrete orientation of the vertices as an $\varepsilon$-length segment that has to be in the cycle.
%This definition would be closer to the geometric interpretation of the problem but the formal definition would be more difficult since $\varepsilon$-segments cannot be expressed by concrete coordinates.
%
% ./figures/cycle_example.eps

%Full coverage
In the full coverage variant, we want a set of cycles (cycle cover) or a single cycle (tour) such that the sum of distance costs and turn costs are minimal and every point $p\in P$ is covered.
\begin{problem}[Full coverage geometric cycle cover]
	Given a set of polygonal obstacles $\mathcal{O}$ in $\mathbb{R}^2$, a set of points $P$ that do not lie within any obstacle, and a function $\delta: P\rightarrow \mathcal{P}( [0, \pi) )$ with $ \forall p\in P: |\delta(p)|\leq \omega$ for some fixed $\omega\in \mathbb{N}^+$.
	Further, the distance cost weight $\kappa\in \mathbb{R}_0^+$ and the turn cost weight $\tau\in \mathbb{R}_0^+$.
	Wanted is a set of cycles $\mathcal{C}=C_0, \ldots, C_m$ that do not intersect $\mathcal{O}$, such that $\sum_{C_i\in \mathcal{C}} c_{\mathcal{O},\kappa, \tau}(C_i)$ is minimal, and every point $p\in P$ is covered by a least on cycle $C_i\in \mathcal{C}$.
\end{problem}
\begin{problem}[Full coverage geometric tour]
	Given a set of polygonal obstacles $\mathcal{O}$ in $\mathbb{R}^2$, a set of points $P$ that do not lie within any obstacle, and a function $\delta: P\rightarrow \mathcal{P}( [0, \pi) )$ with $\forall p\in P: |\delta(p)|\leq \omega $ for some fixed $\omega\in \mathbb{N}^+$.
	Further, the distance cost weight $\kappa\in \mathbb{R}_0^+$ and the turn cost weight $\tau\in \mathbb{R}_0^+$.
	Wanted is a single polygonal cycle $C$ that does not intersect $\mathcal{O}$, such that $c_{\mathcal{O},\kappa, \tau}(C)$ is minimal and every point $p\in P$ is covered.
\end{problem}


%Penalty coverage
In the penalty coverage variant, we want a set of cycles (cycle cover) or a single cycle (tour), such that the sum of distance costs, turn costs, and penalty costs are minimal.
The penalty $\rho(p)$ is added for every point $p\in P$ that is not covered.
\begin{problem}[Penalty geometric cycle cover]
	Given a set of polygonal obstacles $\mathcal{O}$ in $\mathbb{R}^2$, a set of points $P$ that do not lie within any obstacle, a function $\delta: P\rightarrow \mathcal{P}( [0, \pi) )$ with $\forall p\in P: |\delta(p)|\leq \omega $ for some fixed $\omega\in \mathbb{N}^+$, and a penalty function $\rho: P\rightarrow \mathbb{R}^+_0$.
	Further, let $\kappa\in \mathbb{R}_0^+$ be the distance cost coefficient and $\tau\in \mathbb{R}_0^+$ be the turn cost coefficient.
	Wanted is a set of cycles $\mathcal{C}$ for which $\sum_{C_i\in \mathcal{C}} c_{\mathcal{O}, \kappa, \tau}(C)+\sum_{p\in P, \forall C_i \in \mathcal{C}: p\not \in C_i} \rho(p)$ is minimal.
\end{problem}
\begin{problem}[Penalty geometric tour]
	Given a set of polygonal obstacles $\mathcal{O}$ in $\mathbb{R}^2$, a set of points $P$ that do not lie within any obstacle, a function $\delta: P\rightarrow \mathcal{P}( [0, \pi) )$ with $\forall p\in P: |\delta(p)|\leq \omega $ for some fixed $\omega\in \mathbb{N}^+$, and a penalty function $\rho: P\rightarrow \mathbb{R}^+_0$.
	Further, the distance cost weight $\kappa\in \mathbb{R}_0^+$ and the turn cost weight $\tau\in \mathbb{R}_0^+$.
	Wanted is a single polygonal cycle $C$ for which $c_{\mathcal{O}, \kappa, \tau}(C)+\sum_{p\in P, p\not \in C} \rho(p)$ is minimal.
\end{problem}



%Hardness
%With obstacles, a grid graph can be modeled and the NP-hardness of the full coverage geometric cycle cover follows from the NP-hardness of the subset coverage cycle cover problem (in 2-dimensional grid graphs) (Theorem~\ref{th:gg:hard:nphardsubset}).
%As it is contained in all the other problems, all the other problems are NP-hard, too.
%Even without obstacles, we can use the NP-hardness proof for the angular metric cycle cover problem by Aggarwal et al.~\cite{aggarwal2000angular}.


==> 97_nphard.tex <==
\section{Details on NP-Hardness of Minimum-Turn Cycle Cover}
\label{app:A}




==> 98_approximation.tex <==
\section{Details for the Approximation Algorithms}

In this part of the appendix we give additional details on the approximation techniques. 
We provide a detailed proof of Theorem~\ref{th:ccapx} on how to obtain a 12-approximation algorithm for penalty tours in grid graphs (from which the other cases can easily be deduced), and some additional details on the geometric version.

\subsection{Cycle Cover}
\label{sec:app:ccapx}

\statement{Theorem}{th:ccapx}{ \emph{A minimum-weight perfect matching of the endpoints of the dominant {atomic strips} of the fractional solution of the integer program \eqref{eq:ip:obj}-\eqref{eq:ip:inout} yields a $2\omega$-approximation for semi-quadratic (penalty) cycle cover if the edge weights satisfy Eq.~(\ref{eq:triang}).}}
\begin{proof}
\end{proof}

\subsection{Tours}
\label{sec:app:tourapx}




==> Makefile <==
# This is the magic latex makefile composed by Dominik Krupke (krupke@ibr.cs.tu-bs.de) for writing papers.
# You can find the corresponding repository at https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex
# A lot of the ideas are taken and composed from various sources. So feel free to steal it yourself.
-include Makefile.local

# The following variable usually don't need to be altered
TEXFILES:=$(sort $(wildcard *.tex) $(wildcard **/*.tex))

pdf: figures $(TEXFILES)
	latexmk --output-directory=.auxiliary-latex -pdf $(MAIN).tex
	cp ./.auxiliary-latex/$(MAIN).pdf ./$(MAIN).pdf

.DEFAULT_GOAL = all
.PHONY: all check clean

all: pdf

setup: python3
	python3 ./makefile_utils.py --setup

update:
	$(if $(shell command -v wget 2> /dev/null),,$(error Please install `wget` to continue. This should be possible with nearly all package managers. On OS X with Homebrew for example via `brew install wget`))
	wget https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex/raw/master/Makefile -O Makefile
	wget https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex/raw/master/makefile_utils.py -O makefile_utils.py

python3:
	$(if $(shell command -v python3 2> /dev/null),,$(error Please install `python3` to continue. This should be possible with nearly all package managers. On OS X with Homebrew for example via `brew install python`))

figures: python3
	python3 ./makefile_utils.py --svg
	python3 ./makefile_utils.py --ipe

autofix: python3
	python3 ./makefile_utils.py --autofix

check: packagecheck spellcheck grammarcheck phrasingcheck fontcheck texcheck

phrasingcheck: python3
	python3 ./makefile_utils.py --diction $(MAIN).tex --language $(LANGUAGE)

packagecheck: python3
	python3 ./makefile_utils.py --packages

fontcheck: python3
	python3 ./makefile_utils.py --fonts

spellcheck:
	python3 ./makefile_utils.py --spell $(MAIN).tex --language $(LANGUAGE)

grammarcheck: python3
	python3 ./makefile_utils.py --grammar $(MAIN).tex --language $(LANGUAGE)

texcheck:
	python3 ./makefile_utils.py --texlint $(MAIN).tex

clean:
	rm -f $(MAIN).pdf
	rm -rf .auxiliary-latex

showchanges:
ifeq ($(VCS),git)
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		$(VCS) --no-pager diff --color-words $$texfile;\
		done
endif
ifeq ($(VCS),svn)
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		$(VCS) diff $$texfile; \
		done
endif

diff-pdf:
	latexdiff-vc --$(VCS) --flatten -r $(REFERENCE_REVISION) $(MAIN).tex
	latexmk --output-directory=.auxiliary-latex-diff -pdf $(MAIN)-diff$(REFERENCE_REVISION).tex
	cp ./.auxiliary-latex-diff/$(MAIN)-diff$(REFERENCE_REVISION).pdf .
	rm $(MAIN)-diff$(REFERENCE_REVISION).tex


